DORec: Decomposed Object Reconstruction and Segmentation Utilizing 2D Self-Supervised Features

Recovering 3D geometry and textures of individual objects is crucial for many robotics applications, such as manipulation, pose estimation, and autonomous driving. However, decomposing a target object from a complex background is challenging. Most existing approaches rely on costly manual labels to acquire object instance perception. Recent advancements in 2D self-supervised learning offer new prospects for identifying objects of interest, yet leveraging such noisy 2D features for clean decomposition remains difficult. In this paper, we propose a Decomposed Object Reconstruction (DORec) network based on neural implicit representations. Our key idea is to use 2D self-supervised features to create two levels of masks for supervision: a binary mask for foreground regions and a K-cluster mask for semantically similar regions. These complementary masks result in robust decomposition. Experimental results on different datasets show DORec's superiority in segmenting and reconstructing diverse foreground objects from varied backgrounds enabling downstream tasks such as pose estimation.

==> teaser.tex <==
\vspace{0.2cm}
\makeatletter
\let\@oldmaketitle\@maketitle%
\renewcommand{\@maketitle}{\@oldmaketitle%
  \begin{center}
    \includegraphics[width=\linewidth]{figs/teaser4.png}
  \end{center}
  \captionsetup{type=figure}
  \vspace{-0.3cm}
  \captionof{figure}{
  \textbf{Decomposed segmentation and reconstruction}. By leveraging self-supervised 2D features in the form of coarse- and median-grained masks, our proposed method DORec achieves decomposed object reconstruction without 2D annotations and enables downstream tasks.
  }
  \label{fig:teasesr}
 \vspace{-0.63cm}
  }%

